Hardness of Learning DNFs using Halfspaces

The problem of learning $t$-term DNF formulas (for $t = O(1)$) has been studied extensively in the PAC model since its introduction by Valiant (STOC 1984). A $t$-term DNF can be efficiently learnt using a $t$-term DNF only if $t = 1$ i.e., when it is an AND, while even weakly learning a $2$-term DNF using a constant term DNF was shown to be NP-hard by Khot and Saket (FOCS 2008). On the other hand, Feldman et al. (FOCS 2009) showed the hardness of weakly learning a noisy AND using a halfspace -- the latter being a generalization of an AND, while Khot and Saket (STOC 2008) showed that an intersection of two halfspaces is hard to weakly learn using any function of constantly many halfspaces. The question of whether a $2$-term DNF is efficiently learnable using $2$ or constantly many halfspaces remained open. In this work we answer this question in the negative by showing the hardness of weakly learning a $2$-term DNF as well as a noisy AND using any function of a constant number of halfspaces. In particular we prove the following. For any constants $\nu, \zeta > 0$ and $\ell \in \mathbb{N}$, given a distribution over point-value pairs $\{0,1\}^n \times \{0,1\}$, it is NP-hard to decide whether, YES Case: There is a $2$-term DNF that classifies all the points of the distribution, and an AND that classifies at least $1-\zeta$ fraction of the points correctly. NO Case: Any boolean function depending on at most $\ell$ halfspaces classifies at most $1/2 + \nu$ fraction of the points of the distribution correctly. Our result generalizes and strengthens the previous best results mentioned above on the hardness of learning a $2$-term DNF, learning an intersection of two halfspaces, and learning a noisy AND.

==> reg-blocks.tex <==
\section{Analysis for the regular blocks setting}					\label{sec:reg-blocks}

In this subsection, we shall rule out the setting where all the blocks are $\tau$-regular. In particular, we shall prove the following lemma:

\begin{lemma}					\label{lem:reg-block-anticonc}
	Let $\ell = \sum_{v \in e} \Langle c_v,X_v \Rangle + \theta$ be $\tau$-regular i.e, for every vertex $v \in e$ and label $i \in [M]$ we have $\|c_{v,i}\|^2 \leq \tau\|c\|^2$. Additionally, suppose for every vertex $v \in e$, the coefficient vector satisfies $\sum_{i\in [k]}\|c^{(i)}_v\|^4_2 \leq 2\tau\|c_v\|^4_2$. Then we have 
	\begin{equation}
	\Ex_\Lambda\left|\Ex_{X_{\oS} \sim \done|\Lambda,Y_{\oS} \sim \dzero|\Lambda }\left[{\rm pos}\big(\ell(X_\oN,X_\oS)\big) - {\rm pos}\big(\ell(X_\oN,Y_\oS)\big)\right]\right| \leq O(k^{-1/4})
	\end{equation}
\end{lemma}

We setup some notation that will used in the proof of the above lemma. We shall denote by $\oN = (N_1,N_2,\ldots,N_m)$, the choice of noisy rows from each block which are  sampled from Bernoulli distribution. Similarly, we shall denote by $\oS = (S_1,S_2,\ldots,S_m)$ the choice of rows from each block, from which a subset of rows are sampled from $\{e_1,e_2,\ldots,e_q\}$. Finally, let $\oQ = (Q_1,Q_2,\ldots,Q_m)$ denote the choice of indices which are set to $1$ in the rows corresponding to $\oS$.     

Note that the distribution of $(\oN,\oS)$ is identical under distributions $\dzero$ and $\done$. We begin by analyzing the behavior of a single block under distributions $\done$ and $\dzero$. In what follows, we shall use $X_1,X_2,\ldots,X_{2k}$ to denote the $2k$ sets of variables involved in hyperedge $e$, and instead use $(X_{i})_{i \in [2k]} \sim \done$ and $(Y_{i})_{i \in [2k]} \sim \dzero$ to distinguish between whether the random variables are being drawn from the $\done$ or $\dzero$ distributions.

For any label $j \in [m]$, we refer to the restriction of the coefficient vector $c$ to coordinates which project to $j$ as $c^{(j)}$. For any vertex label pair $(v,\alpha)$, the corresponding coefficient is denoted by $c_{v,\alpha}$. Analogously, the restriction of the vertex $v$ to the $j^{th}$ block is denoted by $c^{(j)}_{v}$. 
Throughout the analysis, we shall crucially use the following property of the distributions $\done,\dzero$.

\begin{proposition}
	Fix a hyperedge $e$, and let $\dzero,\done$ denote the $0,1$ distributions restricted to the hyperdge $e$. Then for any vertex $v \in e$, label $j \in [M]$ and coordinate $r \in [q]$,  we have $\Ex_\done[X_{v,j,r}] = \Ex_\dzero[X_{v,j,r}]$. Consequently, for any vertex $v \in e$ we have $\Ex_{X_v \sim \done}\Big[\Langle c_v, X_v \Rangle \Big] = \Ex_{X_v \sim \dzero}\Big[\Langle c_v, X_v \Rangle \Big]$.
\end{proposition}


\subsection{Variance Analysis on a Single Block}

Consider a single block $i \in [m]$, and its associated linear form $\ell(X) = \Langle c^{(i)}, X^{(i)} \Rangle = \sum_{r \in [2k]} \Langle c_r,X_r \Rangle$, where in the last step we drop the indexing by $i$ for brevity, since the entire analysis is on block $i$. 

Note that since the row-wise marginals match under the distribution $\dzero,\done$, for every row $r \in [2k]$ we have $\Ex_{X_r \sim \done} \Langle c_r,X_r \Rangle = \Ex_{Y_r \sim \dzero} \Langle c_r,Y_r \Rangle$, and hence 
\begin{eqnarray*}
\E_{N,S}\Ex_{X \sim \done|(N,S)}\left[\Langle c^{(i)},X^{(i)}\Rangle\right] &=& \E_{N,S}\Ex_{X \sim \done|(N,S)}\left[\sum_{r \in [2k]}\Langle c_r,X_r \Rangle \right] \\
&=& \E_{N,S}\Ex_{X \sim \done|(N,S)}\left[\sum_{r \in N}\Langle c_r,X_r \Rangle \right] + \E_{N,S}\Ex_{X \sim \done|(N,S)}\left[\sum_{r \in S}\Langle c_r,X_r \Rangle \right] \\
&=& \E_{N,S}\Ex_{X \sim \dzero|(N,S)}\left[\Langle c^{(i)},X^{(i)} \Rangle \right] 
\end{eqnarray*}

Since we set the noisy coordinates independent of the choice of distribution $\cD_0$ or $\cD_1$, it follows that 
\begin{equation}
\E_{N,S}\Ex_{X \sim \cD_1|(N,S)}\left[\sum_{r \in N}\Langle c_r,X_r \Rangle \right] = \E_{N,S}\Ex_{X \sim \cD_0|(N,S)}\left[\sum_{r \in [N]}\Langle c_r,X_r \Rangle \right] 
\end{equation}

Therefore combining the two above equations we have that 
\begin{equation}							\label{eqn:S-contrib}
\E_{N,S}\Ex_{X \sim \cD_1|(N,S)}\left[\sum_{r \in S}\Langle c_r,X_r \Rangle \right] = \E_{N,S}\Ex_{Y \sim \cD_0|(N,S)}\left[\sum_{r \in [S]}\Langle c_r,Y_r \Rangle \right] 
\end{equation}

We bound the variance of the difference contribution as follows:
\begin{align}		\label{eq:bound}
&{\rm Var}\Big(\sum_{r \in S} \Langle c_r, X_r \Rangle - \Langle c_r,Y_r \Rangle \Big)\\
&\Ex_{N,S,\oQ}\Ex_{X,Y|N,S}\left[ \left(\sum_{r \in S} \Langle c_r, X_r \Rangle - \Langle c_r,Y_r \Rangle\right)^2 \right]\\
&\overset{1}{\leq} 2\Ex_{N,S}\Ex_{X,Y|N,S} \left[\Big(\sum_{r \in S}\Langle c_r,X_r\Rangle\Big)^2\right] + 2\Ex_{N,S}\Ex_{X,Y|N,S}\left[\Big( \sum_{r \in S}\Langle c_r,Y_r  \Rangle \Big)^2\right]\\
&\overset{1}{\leq} 2\Ex_{N,S}\Ex_{X|N,S} \left[\Big(\sum_{r \in S}\Langle c_r,X_r\Rangle\Big)^2\right] + 2\Ex_{N,S}\Ex_{Y|N,S}\left[\Big( \sum_{r \in S}\Langle c_r,Y_r  \Rangle \Big)^2\right]\\
\end{align}
where in step $1$ we use the fact that $(A - B)^2 \leq 2A^2 + 2B^2$ for any $A,B \in \mathbbm{R}$. We now proceed to bound the first term, the second term can be bounded similarly.
\begin{eqnarray}
\Ex_{N,S,}\Ex_{X \sim \cD_1|N,S} \left[\Big(\sum_{r \in S} \Langle c_{r}, X_{r}\Rangle\Big)^2\right] 
&\overset{1}{\leq}& \Ex_{N,S}\Ex_{X \sim \cD_1|N,S} \sum_{r \in S}\sum_{j \in \pi^{-1}_{v_r}(i)}|S||\pi^{-1}_{v_r}(i)|  \left[\Langle c_{r,j}, X_{r,j}\Rangle^2\right] \label{eq:eqn1}		\\
&\overset{2}{\leq}& 2td \Ex_{N,S} \sum_{r \in S}\sum_{j \in \pi^{-1}_{v_r}(i)}  \Ex_{X \sim \cD_1|N,S}\left[\Langle c_{r,j}, X_{r,j}\Rangle^2\right] 	\nonumber\\
&\overset{3}{\leq}& 2dt\Ex_{N,S} \sum_{r \in S}\sum_{j \in \pi^{-1}_{v_r}(i)} \frac{\|c_{v_r,j}\|^2}{q} \nonumber\\
&=& 2dt\Ex_{N,S} \sum_{r \in S}\frac{\|c_{r}\|^2}{q} \nonumber\\
&\leq& \frac{2dt}{q}\sum_{r \in [2k]} \|c_r\|^2 \Pr_{N,S}\Big[r \in S\Big]		\nonumber\\
&{\leq}& \frac{4dt^2\|c^{(i)}\|^2}{kq}					\label{eq:eqn2}
\end{eqnarray}
where step $1$ follows from Cauchy-Schwarz, step $2$ uses the bounds on $|S|$ and the preimage sizes of the labels. For step $3$, we observe that 
\begin{eqnarray*}
\Ex_{X \sim \cD_1|N,S}\left[\Langle c_{r,j}, X_{r,j} \Rangle^2\right]
&=& \sum_{l \in [q]}\Ex_{X \sim \cD_1|N,S}\left[ c^2_{r,j,l}, X^2_{r,j,l}\right] + \sum_{l_1 \neq l_2}\Ex_{X \sim \cD_1|N,S}\left[c_{r,j,l_1} c_{r,j,l_2}X_{r,j,l_1}X_{r,j,l_2}\right]  \\
&=& \sum_{l \in [q]}\frac{c^2_{r,j,l}}{q} = \frac{\|c_{r,j}\|^2}{q}
\end{eqnarray*}
where in the second equality, we observe that all the cross-terms in the summation are $0$, since at most one of the $X_{r,j,l}$ variables will be set to $1$.
\paragraph{Combining the arguments for the blocks}
Note that the above set of arguments apply to any fixed block $i \in [m]$. Applying Eq. \ref{eqn:S-contrib} to all the blocks we get  

\begin{equation}
\Ex_{\overline{N},\overline{S}}\Ex_{X ,Y | \overline{N},\overline{S}} \left[\sum_{i \in [m]} \Langle c^{(i)}_{S_i}, X^{(i)}_{S_i} - Y^{(i)}_{S_i} \Rangle \right] = 0
\end{equation}

Furthermore by the above analysis for the variance bound we have

\begin{eqnarray}
{\rm Var}\left(\sum_{i \in [m]} \Langle c^{(i)},X^{(i)}_{S_i} - Y^{(i)}_{S_i} \Rangle \right) 
&=& \sum_{i \in [m]}{\rm Var}\left( \Langle c^{(i)},X^{(i)}_{S_i} - Y^{(i)}_{S_i} \Rangle \right) \\ 
&\leq& \frac{8dt^2}{kq}\sum_{i \in [m]}\|c^{(i)}\|^2_2 = \frac{8dt^2}{kq}\|c\|^2_2 
\end{eqnarray}
where the inequality follows by applying the arguments from Eq. \ref{eq:eqn1}-\ref{eq:eqn2} to both the $X$ and $Y$ terms from Eq. \ref{eq:bound}. Finally, using Chebyshev's inequality, we have 
\begin{equation*}
\Pr_{X,Y,N,S}\left[\left| \sum_{i \in [m]} \Langle c^{(i)}_{S_i},X^{(i)}_{S_i} - Y^{(i)}_{S_i} \Rangle \right| \geq \frac{8dt}{qk^{1/4}}\|c\|\right] \leq\frac{2}{k^{1/4}}
\end{equation*}


\subsection{Anti-concentration from the noisy blocks}					\label{sec:anti-conc}

	The anti-concentration step here relies on the Berry-Esseen theorem. We prove it for the distribution $\done$, the proof for distribution $\dzero$ is identical.
	
	Recall that from the setting of Lemma \ref{lem:reg-block-anticonc} for every vertex $v \in V$, and block $i \in [m]$ we have $\|c^{(i)}_{v}\|^2 \leq \|c_v\|^2$.  Also recall that for any $i \in [m]$, $N_i$ denotes the set of rows which will be sampled from the Bernoulli Distribution. 
	
	We will begin by fixing a realization of $(N,S)$. Let $\cI = \cup_{i \in [m]} \cup_{v \in N_i} \{v\} \times \pi^{-1}_{v}(i)$ denote the set of all point label pairs for which the variables in $X_{v,j}$ will be drawn from the Bernoulli distribution. Recall that For every $i\in[m]$, the coordinates in $X^{(i)}_{N_i}$ are sampled independently with probability $\frac12$. 
	
	For every $(v,j) \in \cI$ and $r \in [q]$, define random variable $Z_{v,j,r} = c_{v,j,r}\left(X_{v,j,r} - \frac12\right)$. Then by definition, for every such $(v,j) \in \cI$ we have 
	\begin{eqnarray}						\label{eqn:2nd-moment}
	\E\Big[Z^2_{v,j,r}\Big] &=& \Ex\left[c^2_{v,j,r}\left(X_{v,j,r} - \frac12\right)^2\right] = \frac{c^2_{v,j,r}}{4}
	\end{eqnarray}
	Furthermore, again for every $(v,j,r) \in \cI \times [q]$, denote by $\sigma^2_{v,j,r} := \E Z^2_{v,j,r}$ and define the random variable $\tilde{Z}_{v,j,r} = Z_{v,j,r}/\sigma$ where $\sigma := \sqrt{\sum_{(v,j) \in \cI} \sum_{r \in [q]} \sigma^2_{v,j,r}}$. 
	Plugging in Eq. \ref{eqn:2nd-moment} we get 
	\begin{eqnarray}
	\sigma^2 = \sum_{i \in[m]}\sum_{v \in N_i}\sum_{j \in \pi^{-1}_v(i)} \Ex Z^2_{v,j} 
	&=& \sum_{i \in[m]}\sum_{v \in N_i}\sum_{j \in \pi^{-1}_v(i)} c^2_{v,j}\\
	&=& \sum_{i \in[m]}\sum_{v \in N_i}\|c^{(i)}_v\|^2\\
	&=& \sum_{i \in[m]}\|c^{(i)}_{N_i}\|^2 
	\end{eqnarray}
	Then by definition we have (i) $\E \tilde{Z}_{v,j,r} = 0$ (ii) $\sum_{i \in[m]}\sum_{(v,j)} \sum_{r \in [q]} \E \tilde{Z}^2_{v,j} = 1$, and (iii) we can bound the sum of the third moments as 
	\begin{eqnarray}
	\E \sum_{(v,j) \in \cI}\sum_{r \in [q]} \Big[|\tilde{Z}_{v,j,r}|^3\Big]
	&\leq&  \max_{(v,j) \in \cI, r\in [q]}\|Z_{v,j,r}\|_{L_\infty}  \E \sum_{(v,j) \in \cI}\sum_{r \in [q]} \Big[ |\tilde{Z}_{v,j,r}|^2\Big] \\
	&\leq& \max_{(v,j) \in \cI,r \in [q]} \frac{\|Z_{v,j,r}\|_{L_\infty}}{\sigma} \\
	&\leq& \max_{(v,j) \in \cI} \frac{\|c_{v,j}\|}{\sigma} \\
	&\leq& \tau^{1/2}\frac{\|c\|}{\sigma}
	\end{eqnarray}
	Therefore using Berry Esseen Theorem, for finite interval $I \subset \mathbbm{R}$ we have  
	\begin{equation}
	\Pr \left[\sum_{(v,j,r) \in \cI \times [q]} \tilde{Z}_{v,j,r} \in I\right] \leq O(\tau^{1/4}) + \Pr_{g \sim N(0,1)} \Big[g \in I\Big] \leq O\left(\tau^{1/2}\frac{\|c\|_2}{\sigma}\right) + |I|
	\end{equation}
	Rolling back the sequence of variable transformations we get that,
	\begin{equation}
	\sum_{(v,j,r) \in \cI \times [q]} \tilde{Z}_{v,j,r} \in I \iff \sum_{(v,j,r) \in \cI \times [q]} Z_{v,j} \in \sigma I \iff \sum_{i \in [m]} \Langle c^{(i)}_{N_i},X^{(i)}_{N_i} \Rangle \in \sigma I + \sum_{i \in [m]} \Langle c^{(i)},\frac12\vone \Rangle 
	\end{equation}
	Therefore, for a fixed choice of $(\oN,\oS)$ for any interval $[\alpha,\beta] \subset \mathbb{R}$ we have 
	\begin{equation}				\label{eqn:anti-conc}
	\Pr_{X_{\oN}}\Big[\Langle c_{\overline{N}},X_{\overline{N}} \Rangle \in [\alpha,\beta] \Big] \leq O(\tau^{1/4}) + \frac{|\alpha - \beta|}{\sigma}  
	\end{equation}
	To complete the proof, using arguments identical to the ones used in Lemma \ref{lem:anti-conc-2}, we get the following high probability lower bound on $\sigma$. 
	\[
		\Pr\left[\sum_{v \in e} \left\|c^{N(v)}_v\right\|^2 \leq \frac{\|c\|^2}{8}\right] \leq \Pr\left[ \exists v \in e : \left\|c^{N(v)}_v\right\|^2 \leq \frac{\|c\|^2}{8} \right] \leq 2k\exp\left(-\frac{1}{32\tau}\right) 
	\] 
	Therefore, with probability at least $1 - e^{-\Omega(1/\tau)}$, we have $\sigma^2 = \sum_{v \in e}\|c^{N(v)}_{v}\|^2 \geq \frac18\|c\|^2$. Combining the tail bound with Eq. \ref{eqn:anti-conc} we get
	\begin{equation}
	\Pr_{\oN, X_{\oN}}\Big[\Langle c_{\overline{N}},X_{\overline{N}} \Rangle \in [\alpha,\beta] \Big] \leq O(\tau^{1/4}) + O(|\alpha - \beta|)
	\end{equation}
	which gives us the required anti-concentration bound.

	\subsection{Proof of Lemma \ref{lem:reg-block-anticonc}}				\label{sec:alys-reg-form}

	Recall that the random variable $(\oS,\oN)$ is distributed identically under $\done,\dzero$. Now we observe the following.  
	
	\begin{itemize}
		\item Using the arguments from Section \ref{sec:anti-conc}, we know that with probability at least $1 - 100/k^{1/4} - O(\tau^{1/4})$ over the choice of $\oN, X_{\oN}$, we have $|\Langle c_{\overline{N}},X_{\overline{N}}\Rangle  + \theta | \geq \frac{50}{k^{1/4}}$
		\item With probability at least $1 - \frac{1}{k^{1/4}}$ (over the choice of $\oS,\oN,X_{\oS},Y_{\overline{S}}$) we have $|\Langle c_{\overline{S}}, X_{\overline{S}} - Y_{\overline{S}} \Rangle | \leq \frac{1}{k^{1/4}}$.
	\end{itemize}
	Combining the above arguments we have
	\begin{align*}
	&\Ex_{\oN,\oS}\Ex_{X_\oN}\left|\Ex_{X_\oS \sim \done |\oS, {Y_\oS \sim \dzero |\oS} } \left[{\rm pos}\Big(\Langle c_{\oS} , X_{\oS} \Rangle + \Langle c_{\oN} , X_{\oN} \Rangle + \theta \Big)\right] - \left[{\rm pos}\Big(\Langle c_{\oS} , Y_{\oS} \Rangle +\Langle c_{\oN} , X_{\oN} \Rangle +  \theta \Big)\right] \right| \\ 
	&\leq \Ex_{\oN,\oS}\Ex_{X_\oN}\left|\Ex_{X_\oS \sim \done |\oS, Y_\oS \sim \dzero|\oS} \left[\mathbbm{1}\Big( {\rm pos}\left(\Langle c_{\oN},X_\oN \Rangle + \Langle c_{\oS},X_{\oS} \Rangle + \theta\right) \neq {\rm pos}\left(\Langle c_{\oN},X_\oN \Rangle + \Langle c_{\oS},Y_{\oS} \Rangle + \theta\right)\Big)\right] \right| \\ 
	&\leq \Ex_{\oN,\oS}\Ex_{X_\oN}\Ex_{X_\oS \sim \done|\oS,Y_\oS \sim \dzero|\oS}\left[\mathbbm{1}\Big(\left|\Langle c_\oN,X_\oN \Rangle + \theta \right| < \left| \Langle c_{\oS},X_\oS - Y_{\oS} \Rangle \right|\Big)\right] \\
	&\leq \Ex_{\oN,\oS}\Ex_{X_\oN}\Ex_{X_\oS \sim \done|\oS,Y_\oS \sim \dzero|\oS}\left[\mathbbm{1}\left(\left\{\left|\Langle c_\oN,X_\oN \Rangle + \theta \right| < \frac{10}{k^{1/4}} \right\} \bigvee \left\{ \left| \Langle c_{\oS},X_\oS - Y_{\oS} \Rangle \right| > \frac{10}{k^{1/4}}\right\}\right)\right] \\
	& \leq O(k^{-1/4})
	\end{align*}

